Ducho: A Unified Framework for the Extraction of Multimodal Features in Recommendation

In multimodal-aware recommendation, the extraction of meaningful multimodal features is at the basis of high-quality recommendations. Generally, each recommendation framework implements its multimodal extraction procedures with specific strategies and tools. This is limiting for two reasons: (i) different extraction strategies do not ease the interdependence among multimodal recommendation frameworks; thus, they cannot be efficiently and fairly compared; (ii) given the large plethora of pre-trained deep learning models made available by different open source tools, model designers do not have access to shared interfaces to extract features. Motivated by the outlined aspects, we propose \framework, a unified framework for the extraction of multimodal features in recommendation. By integrating three widely-adopted deep learning libraries as backends, namely, TensorFlow, PyTorch, and Transformers, we provide a shared interface to extract and process features where each backend's specific methods are abstracted to the end user. Noteworthy, the extraction pipeline is easily configurable with a YAML-based file where the user can specify, for each modality, the list of models (and their specific backends/parameters) to perform the extraction. Finally, to make \framework accessible to the community, we build a public Docker image equipped with a ready-to-use CUDA environment and propose three demos to test its functionalities for different scenarios and tasks. The GitHub repository and the documentation are accessible at this link: https://github.com/sisinflab/Ducho.

==> src/framework_backup.tex <==
\section{Architecture}
% not final
% it clearly needs correction and changes dont worry i'll deal with it 

\framework is built around three main components: Dataset, Extractor, and Runner. Other classes are utilized to support them; the most important one is the Config class. The architecture is designed to be modular, allowing for adding new functionalities by implementing and replacing components. This section will discuss these main components; later, we will discuss the Config class because, although it is not a main component, it is essential for the workflow, and in case of customization, it will probably need to modify as well. Before proceeding, it is essential to note that \framework is a Multimodal Feature Extraction library, and each type of extraction works differently. There is not just one Extractor or Dataset but three different types of each, depending on the type of extraction. Understanding how each works is unnecessary, as they share the same interface. The following sections will provide a description and purpose of all the main components of \framework.
\subsection{Dataset}
The Dataset class is one of the three main components of \framework. Its purpose is to manage the data given in input by the user to elaborate and create the output file. The Dataset class will also preprocess the data  before giving it to the Extractor class that will later execute the feature extraction with those data. There is not a general Dataset class, but three kind, one for each type of data: VisualDataset, TextualDataset, AudioDataset. Since this three classes share the same interface, all of them are inheritance of the same DatasetFather class. The Dataset classes needs in input the absolute path of the folder where the files are,
except for TextualDataset that needs in input 
% it is important to notice that only the TextualDatase needs in input
the absolute path to the file where the entries
are.
% OPTIONAL
%Anyway when writing the configuration info in the config file, there is no need to give the absolute path of the file to elaborate, infact that absolute path is built adding the dataset folder (from the dataset entry) with the relative folder path of the samples. This subject will be described thoroughly in the section of the configuration file.

To execute the preprocessing additional information are needed. These information must be written in the model section since each model may need different preprocessing infos (see the \Cref{sec:dict} for additional information). The preprocessing done is:
\begin{itemize}
    \item Cleaning text, for textual extraction.
    \item Resize and Normalization of the image, for visual extraction.
    \item Re-sample of the audio wave, for audio extraction.
\end{itemize}

The retrieving of the data for extraction is done by the Dataset exposing the method \emph{get\_item}: which given an index, preprocesses the indicated contents and returns them.
 A cycle in Runner elaborates all the input data, finally after the extraction, the dataset will be reused to write the output in a numpy file using the method \emph{create\_output\_path}.
 
\subsection{Extractor}
The Extractor class is one of the three main components of \framework. It aims to build a model from a backend framework and execute the feature extraction on a given sample. As said earlier, there is no general Extractor class, but three kinds, one for each data type: VisualExtractor, TextualExtractor, and AudioExtractor. Although they all expose the same call of methods, they all work in very different ways; it is essential to remember that as the Dataset, they all are an inheritance of the same ExtractorFather class. The Extractors use three different libraries: a PyTorch, TensorFlow, and Transformers (from  Hugging Face), but not each type of Extractor has all of them: 
\begin{itemize}
    \item VisualExtractor uses Tensorflow and Torchvision.
    \item TextualExtractor uses Transformers and Sentence\_Transformers.
    \item AudioExtractor uses Torchaudio and Transformers.
\end{itemize}
\par
For each extraction, it is possible to use every model the previously cited libraries expose. 
The Textual extraction is an exception: it is needed, with the model's name, to indicate also the task the model has to execute, but if the model were not pre-trained on that task, the default model would be used instead.
%Just a note: in case of the Textual extraction it is needed, with the name of the model to use, also the task you want the model to execute; warning: if that model was not pretrained for that task, the default model for that task will be initialized ( see Transformers Pipeline for more details ). 
%Instead in case of the Audio extraction all the models that you intend to use are trained in ‘from wav to vec’.

In the end, this is how the extractor works: it needs first to set the framework to use, then the model ( as a string, it will instantiate on its own), and finally, with the call of \emph{extract\_feature}, the extraction will start. This last method will need the layer to extract and the sample to use, which was already pre-processed from the Dataset class.




\subsection{Configuration}
% In the end the Config class manage the configuration dictionary, where all the information to execute the extraction are written. This dictionary can be built from a YAML file or given to the framework by a command, the Config class then cleans possible human made errors from the dictionary. After the Config class saves the data whit-in itself and, when asked by the Runner, it returns the needed information. 
%If you intend to modify Ducho, in particular if you intend to change the how the config dict works, remember to modify the right part of this class as well. Whit this in mind we can understand the the core purpose of the Config class is to rework the config info in a way that makes them easily accessible to the rest of the framework, enabling also to change how ther are given or made, in a comfortable way.
% In case of personalization of \framework, if the changes affect the configuration dictionary, the Config class will be modified as well. With this in mind we can understand that the core purpose of the Config class is to rework the config info in a way that makes them easily accessible to the rest of the framework, enabling also to change how they are given or made, in a comfortable way.
The Config class manages the configuration dictionary, where all the information to execute the extraction is written. This dictionary can be built from a YAML file or given to the framework by a command, and the Config class then cleans possible human-made errors from the dictionary. After the Config class saves the data whit-in itself and, when asked by the Runner, it returns the needed information.
In case of customization of \framework, if the changes affect the configuration dictionary, the Config class will also be modified. With this in mind, we can understand that the core purpose of the Config class is to rework the config info in a way that makes them easily accessible to the rest of the framework, enabling them to change how they are given or made comfortably.

\subsection{Runner}
This component is the project's core; using an architecture client/server, it calls and manages all the other components of \framework. It first calls the Config class to know which extractions must be done.
For an exceptional case where only a type of extraction is needed, the Runner exposes three methods to execute only the designed type. Otherwise, the \emph{execute\_extractions} method executes everything described by the Config class. To execute the extraction, the Runner class instantiates the Dataset and the Extractor, and for each model, it sets them the needed information. After that, for each sample data:(i) retrieves the data from the Dataset,(ii) executes the extraction with the Extractor,(iii) gives the output to the Dataset again that will write it in a numpy file.


==> src/pipeline_backup.tex <==
\section{Extraction pipeline}
% how it is expected to interact with ducho
% what input does it needs and what outputs does it gives you

\input{figure/application.tex}

\subsection{Input for configuration}
Since Ducho allows for different types of extractions, it needs a very precise configuration system that tells it what to do. In this section will be described the two ways to give it such information. There are mainly two routes, the first is by giving Ducho a configuration YAML file, the second is giving the dictionary of instruction directly to the Runner class. Anyway to manage the framework easily there is also another option: to use a precompiled file YAML and modify the needed entries from command line.
\subsection{Dictionary's structure}
\label{sec:dict}
In this section there will be a short description of the way to write the dictionary of configurations and use it. It  has two main entries for the setup and then more entries for describe models and preprocessing to actuate.
\par
These first two entries are \emph{dataset\_path}, which describe the path where all the I/O are going to be. While the second entry is the \emph{gpu\_list} where is described the list of GPU that are intended to use. In case the execution will be made on the CPU only, then this entry will have to have the \emph{-1} value
\par
The others entries are needed to describe which model use with which kind of extractions and what preprocessing actuate.
The First is the type of extraction, that defines the type of files to utilize in the extraction, as such it could be \emph{visual}, \emph{textual} or \emph{audio}.
%First let's remember that there are three kind of extraction: \emph{visual}, \emph{textual}, \emph{audio}. 
Each of them can work differently depending on the origin of the data: from \emph{items} or \emph{interactions}. So when describing how a set of model have to work, the entries have to be build in this way as nested dictionaries: 
\par
 First the kind of extraction(i), then the origin of data (ii).  Here (iii) have to be indicated the \emph{input\_folder}(iii.1) and \emph{output\_folder}(iii.2), both relative to the \emph{dataset\_path}. After, in the same location, have to be put the list of models it is intended to execute(iii.3). Each entry of this list is another dictionary which describes the name of the model, the framework, the layers of the model where execute the extraction and others info for the preprocessing that changes with each kind of extraction:
\begin{itemize}
    \item visual: \emph{reshape}, a tuple to describe the height and width of the image reshaping
    \item textual: \emph{clear\_text} to clean the string before extraction
\end{itemize}
\par
Audio in this moment doesn't need this kind of personalization although the logic for future improvements it's added. Finally, the last thing worth mentioning is that the model's dictionary in the textual extraction exposes another flag which is the task that the model will accomplish.
\subsection{Setting the configuration}
As said earlier building a YAML file is not the only way to describe what Ducho has to do, it may be preferable in same cases to give such information directly to the runner through a dictionary. This could be done during the instantiation of the Runner class, using the variable \emph{argv} that will overwrite the config dictionary entirely or partially.
%\subsubsection{How to change an entry in the dictionary}
%As said the argv is used to overwrite a config dictionary, it is a list of tuples key value where each entry is a String that needs to be write in this way: \emph{'key=value'}. 

%The key is used also to describe the path in the dictionary to follow beacuse as described earlier the config dictionary is built of other neted dictionary.
As the config dictionary is built of other nested dictionaries, the key is used also to describe the path within to follow, to do so the '.' is used as a discerning. I.e 'key1.key2.key3'
% THE FOLLOWING CAN BE ELIMINATED SINCE IS DISCUSSED IN THE README OF THE PROJECT
%\subsection{the pipeline}
%To understand how the pipeline works, there is need to describe what input file are expected and what output file will be created. Instead the description of the workflow is futile since the reader can easily understand it by reading the architecture.
\subsubsection{The expected Input and Output file}
\par
The expected Input file for each kind of extractions are:
\begin{itemize}
    \item Visual: it does support every extension supported by Pillow Image
    \item Audio:  it does support every extension supported by torchaudio
    \item Textual: it uses \emph{only one} file per extraction as a tsv
\end{itemize}
\par
The output is always a npy file containing the feature extracted. The path to the file is the output folder given to the config dict and then others folder for each framework and model in cascade.

==> src/pipeline_backup_backup.tex <==
\section{Extraction pipeline}
% how it is expected to interact with ducho
% what input does it needs and what outputs does it gives you

\input{figure/application.tex}

The execution starts from the Runner class, it is the orchestrator of all the other components and will manage them. At the beginning when calling the Runner it is needed to give it the source of Configuration that could be: the path to a Yaml file, a new configuration dictionary or the path to a Yaml file and the changes to overwrite.
The Runner with this information calls the Dataset and ask it to load the input file and pre-process them as described in the configuration. The Dataset returns to the Runner the input file, then the Runner asks the Extractor to Build the model, gives it the input and tells it the layer where to stop to do the extraction. The Extractor execute the feature extraction as per instruction and returns a npy-array; this output is collected by the Runner, who delivers it to the Dataset that writes the output in its designated file.
%ALL THE FOLLOWING HAs TO BE DELETED
%\subsection{Configuration Input}
%Since Ducho allows for different types of extractions, it needs a very precise configuration system that tells it what to do. In this section will be described the two ways to give it such information. There are mainly two routes, the first is by giving Ducho a configuration YAML file, the second is giving the dictionary of instruction directly to the Runner class. Anyway to manage the framework easily there is also another option: to use a precompiled file YAML and modify the needed entries from command line.
%\subsection{Dictionary's structure}
%\label{sec:dict}
%In this section there will be a short description of the way to write the dictionary of configurations: it  has two main entries for the setup and then more entries to describe models and preprocessing to actuate.
%\par
%These first two entries are \emph{dataset\_path}, which describe the path where all the I/O are going to be. While the second entry is the \emph{gpu\_list} where is described the list of GPU that are intended to use. In case the execution will be made on the CPU only, then this entry will have to have the \emph{-1} value.
%\par
%The others entries are needed to describe which model to use with which kind of extractions and what preprocessing actuate.
%The first is the type of extraction, that defines the type of files to utilize in the execution, as such it could be \emph{visual}, %\emph{textual} or \emph{audio}.
%The second is the origin of elaboration, it defines if the data contained in the files describes an item or the interaction of users to items, as such it could assume values as \emph{items} or %\emph{interactions}.
%The last entry to describe is the list of models: it describes which model use and what preprocessing make, each element of the list is a complex dict composed of:
%\begin{description}
    %\item[model name:] is the name of the model. If the backend used is Transformers from huggingface, this name could also indicate the repo of the model as a path (E.g. 'Repo/modelName'). This permits to use personalized models.
    %\item[backend:] are the external libraries used to build the models, such libraries are: \emph{PyTorch}, \emph{TensorFlow} and \emph{Transformers}.
    %\item[list of output layers:] indicates the layers where stop the execution and do the extraction, it is a list of element that could be both Strings or Integer as the model architecture calls them.
%\end{description}
%Another component that belong to the elements of the models list is the preprocessing flag which explains what kind of preprocessing make, these flags change with the type of extraction and are:
%\begin{description}
    %\item[reshape] for \emph{Visual extraction}, is a tuple of width and height as Integer used to reshape the image in a size acceptable by the model
    %\item[clear\_text] for \emph{Textual extraction} is a Boolean flag that describes if the text needs to be cleaned
    %\item[task] for \emph{Textual extraction} is the task that the model will execute during the extraction, if the model is not pre trained on such task, the default model will be used instead. The list of tasks is available \href{https://huggingface.co/docs/transformers/main_classes/pipelines#transformers.pipeline.task}{here} 
%\end{description}



%\subsection{Setting the configuration}
%As said earlier building a YAML file is not the only way to describe what Ducho has to do, it may be preferable in same cases to give such information directly to the runner through a dictionary. This could be done during the instantiation of the Runner class, using the variable \emph{argv} that will overwrite the config dictionary entirely or partially.
%\subsubsection{How to change an entry in the dictionary}
%As said the argv is used to overwrite a config dictionary, it is a list of tuples key value where each entry is a String that needs to be write in this way: \emph{'key=value'}. 
%The key is used also to describe the path in the dictionary to follow beacuse as described earlier the config dictionary is built of other neted dictionary.
%As the config dictionary is built of other nested dictionaries, the key is used also to describe the path within to follow, to do so the '.' is used as a discerning. I.e 'key1.key2.key3'
% THE FOLLOWING CAN BE ELIMINATED SINCE IS DISCUSSED IN THE README OF THE PROJECT
%\subsection{the pipeline}
%To understand how the pipeline works, there is need to describe what input file are expected and what output file will be created. Instead the description of the workflow is futile since the reader can easily understand it by reading the architecture.
%\subsubsection{The expected Input and Output file}
%\par
%The expected Input file for each kind of extractions are:
%\begin{itemize}
%    \item Visual: it does support every extension supported by Pillow Image
%    \item Audio:  it does support every extension supported by torchaudio
%    \item Textual: it uses \emph{only one} file per extraction as a tsv
%\end{itemize}
%\par
%The output is always a npy file containing the feature extracted. The path to the file is the output folder given to the config dict and then others folder for each framework and model in cascade.
